Advancing Earth Observation: A Survey on AI-Powered Image Processing in Satellites

Advancements in technology and reduction in it's cost have led to a substantial growth in the quality & quantity of imagery captured by Earth Observation (EO) satellites. This has presented a challenge to the efficacy of the traditional workflow of transmitting this imagery to Earth for processing. An approach to addressing this issue is to use pre-trained artificial intelligence models to process images on-board the satellite, but this is difficult given the constraints within a satellite's environment. This paper provides an up-to-date and thorough review of research related to image processing on-board Earth observation satellites. The significant constraints are detailed along with the latest strategies to mitigate them.

==> Sections/Applications.tex <==
% \newpage
% \section{Related Work} \label{RelatedWork}
% \subsection{Machine Learning on-board Satellites}


\section{Applications} \label{Applications}
\IEEEPARstart{T}{his} section details the various applications that would benefit from on-board image processing.
\subsection{Disaster Management (Forrest Fire, flood, earthquake) }
The high-resolution images captured by an Earth’s observation satellite often exceed 10 GB. So trying to download this volume of data can adversely affect the speed of response to emergencies such as fires and earthquakes. Processing the data on board would drastically improve this time delay and create a much more time effective response.
\par As early as 2004 Visser et al. \cite{visser2004real} investigated this idea, proposing the use of a high-resolution imaging sensor on board a satellite with a  high processing capacity for detecting and monitoring natural disasters in real time and relaying the information directly to interested parties.
\par Preprocessing images captured from a satellite is the 1st significant task to correct radiometric distortions, atmospheric distortion and geometric distortions present in the raw image data. This is well described by Sowya et al. \cite{sowmya2017remote}. To facilitate on-board processing these tasks have to be optimised. In 2009 Du et al \cite{du2009fast} proposed a method of speeding up the real-time implementation of several popular detection and classification algorithms for image data with different formats. In 2017 Li et al. \cite{li2019fpga} introduced a new FPGA-based implementation spectral unmixing volume calculation formula, fast enough to facilitate real time processing.  
In 2018 Qi et al. \cite{qi2018board} published a paper on doing on-board, real-time image preprocessing of optical remote-sensing imagery to reduce the bottleneck in associated applications such as disaster management. The 1st step was to a optimise a mapping methodology for the preprocessing algorithm. The 2nd part was the design of a parallel acceleration architecture for real-time requirements based on a FPGA and DSP coprocessor.

\subsection{Marine Analysis (fish movement, ship detection, hydrology}
Maritime Surveillance has become a huge challenge, specifically in regions where maritime traffic represents a major economic interest. It's critical to the effective understanding of activities in the maritime domain that could impact on the security, safety and environment of sovereign countries. It can involve detection of patterns of illegal behaviour at sea such as illegal fishing, drug-traffic, smuggling, immigration \& piracy but also ship detection, classification and identification (for cooperative and non-cooperative vessels) for the purpose of enforcing of traffic rules and restricted areas. Environmental impacts include pollution monitoring such as plastic pollution \& oil spills. In 2011 Bocheret \cite{borchert2011future} outlines the complex challenges and opportunities within the domain. Efforts to obtain real time detailed maritime information were made in the 1950s through the introduction of ground-based maritime radars. The automatic identification system (AIS) which is a short-range coastal tracking system was introduced in the 1990's with a similar objective to identify and locate ships. However these do provide a complete coverage of the entire global maritime space so satellite based sensor technologies such as satellite AIS data and synthetic aperture radar (SAR) are used to complement the existing terrestrial technologies. Soldi et al.  \cite{soldi2021space} gives a really through account of these technologies and how they operate to provide near real time data. To provide truly real time information the processing of the imagery has to be done as close to where the data is caputered and in this case this is on the satellite. The same authors carried out a follow on report \cite{soldi2021space} investigating this. 
\par In 2018 a paper \cite{arechiga2018onboard} was published that proposed a new 2 step approach for ship detection from on-board a SmallSat. Step 1 was to use a traditional computer vision technique to detect all objects on the ocean surface. For step 2, a modern CNN (a slimmed down version of VGGnet) would be used to classify the objects as ships or not. The CNN was trained on a Planet Open California dataset containing 2800 images. Tests were carried our using a Nvidia Jetson TX2 (SoC device), with various TX2 modes and test image resolutions. The approach successfully identified all ships along with a few false positives. A comparison of the results were made with the main performance metric being the speed of algorithm execution. The 1st part (ie detecting the objects) took less than 2.5 seconds whereas the 2nd part (classifying objects) took over 30 seconds. On average the neural network required 6.71 ms to classify one 80x80x3 image chip as containing a ship or not. Processing an image containing 6310 ships took 53.9secs which was considered successful as a proof-of-concept that advanced onboard processing applications are possible with the use of a COTS embedded computer such as a TX2 that meets the SWaP (Size, Weight and Power) requirements of a SmallSat. 
% In 2020 Willburger et al. \cite{willburger2020amaro}
In early 2022 Liu et al. \cite{liu2022multi} proposed a lightweight multi ship real-time detection network based on the YOLOv4-LITE model achieving a mean average precision (mAP) of 95\% processing SAR images at 47 frames per second (FPS) and the model size is only 49MB.

\subsection{Land Analysis (cover change, crop health, agriculture, mining)}
\par In March 2021 McBee et al. \cite{mcbee2021considerations} presented the results of the implementation of ML techniques on computationally-constrained, high-reliability spacecraft hardware. One of the test cases involved classifying features of the Earth's surface using the MobileNetV2 CNN trained on satellite imagery data. The hardware used included the RAD5545 which is a radiation hardened single board computer, the LEON3FT is a fault-tolerant processor based on the SPARC V8 architecture, the radiation tolerant PolarFire FPGA and the NVIDIA TX1 is a high performance GPU. The FPGA had the highest throughput with all having simular accuracy results.


\subsection{Other (Weather, novelty (cloud)  }
In late 2018 Zhang et al. \cite{zhang2018cubesat} introduced a new framework for detecting clouds from on-board a satellite. The goal was to reduce the volume of data that needs to be transmitted to ground by automatically removing images with clouds and shadow which can be up to 66\% of the content. Images are first compressed using JPEG2000 on a FPGA processor. Then 4 different CNNs are used to detect the images with clouds on an ARM processor. 
\begin{itemize}
    \item U-Net is a CNN that evolved from the idea of a fully convolutional network \cite{ronneberger2015u}.
    \item MobUNet is a lightweight version of U-Net.
    \item Deconv-Net is based on idea of a deconvolution network \cite{zeiler2010deconvolutional}.
    \item MobDeconv-Net which is a lightweight version of Deconv-Net.
\end{itemize}
The Landsat dataset SPARCS (Statewide Planning and Research Cooperative System) was used for model training and tested (80/20 split) using the Google Cloud Platform. All were deployed in Windows-based TensorFlow environment with a single NVIDIA GTX1060 GPU. Comparisons were made in terms of iteration time during training, training losses, classification accuracy, inference speed \& peak working memory usage.\newline
The MobUNet was judged as the best performer of the CNNs, achieving a classification accuracy of over 93\%, while its maximum memory usage was only 0.71 Mb and the inference speed was 0.038 sec/million pixels.

\par In September 2020 a paper was published \cite{reiter2020fpga} with an approach to create a real-time, remote-sensed cloud detection solution, using a binarized CNN (called CNV-W1A1) on a FPGA platform (Xilinx Zynq-7000 SoC). The highly compressed network achieved an impressive inference throughput of 358.1 images per second with a maximum power consumption of 2.4 W. This throughput was 68 times faster than alternate algorithmic tested previously, and approximately 115 times faster than the CloudScout deep neural network. While the throughput was very high the accuracy of 64\% is comparatively low and maybe unacceptably low depending on the application requirements. 
%The idea of using lower precision, quantized and binary variants of models is one that has shown potential.\cite{courbariaux2016binarized}

\par In November 2020 a lightweight CNN architecture called CubeSatNet was published \cite{maskey2020cubesatnet} as part of the BIRDS-3 project \cite{birds_3_project_2021} from Kyushu Institute of Technology, Japan, with the motivation being to reduce the time and effort in downloading and post-processing, by filtering the data before transmitting it to the ground. It was trained on a new dataset created from combining images freely available from the web, their own small satellite image database, images extracted from live feed of International Space Station along with thumbnail images from Sentinel 3A (satellite owned by ESA). The network is small enough to run on an ARM Cortex microcontroller and has a memory footprint of just 104 kB. The platform is on a very tight power budget with the solar panels generating just 1480 mWh per orbit. It was successfully launched on February 2021 on-board a 1U satellite called BIRDS-4 and is operational at the time of writing. 
Another very recent example where machine learning was used for on board image processing is in the enabling of Autonomous Optical Navigation (OpNav) on board the Milani \cite{pugliatti2023design} which is a 6U CubeSat built as part of Hera mission due to launch in October 2024.



==> Sections/Methodology.tex <==
\section{Methodology}
TBD

==> Sections/Results_and_Analysis.tex <==
\section{Results}
TBD

==> acro_list.tex <==
\begin{acronym}[MPC] % Give the longest label here so that the list is nicely aligned
\acro{ML}{Machine Learning}
\acro{TLA}{Three Letter Acronym}
\end{acronym}
